Theoretical Analysis of Sequential Importance Sampling Algorithms for a Class of Perfect Matching Problems

This paper analyzes the performance of sequential importance sampling algorithms for estimating the number of perfect matchings in bipartite graphs. Precise bounds on the number of samples required to yield an accurate estimate are derived. In doing so, moments of permutation statistics are computed using generating functions and nonstandard limit theorems are derived by expressing perfect matchings as a time-inhomogeneous Markov chain.

==> algorithm.tex <==
% chktex-file 3
\noindent Diaconis~\cite{dia18} proposed the following sampling algorithm for generating a random perfect matching of a bipartite graph $G = ([n], [m'], E)$.
\begin{algorithm}\label{alg:sequential}
  Let $v_1, \ldots, v_n$ be an enumeration of the vertices in $[n]$. Beginning at $v_1$ and proceeding in order:
  \begin{itemize}
    \item
      Check each edge coming out of $v_1$ to see if its removal, and the subsequent removal of the adjacent vertices, leaves a graph allowing a perfect matching. Let $J_1$ be the set of available edges. Pick $e \in J_1$ uniformly and delete this edge.
    \item
      Repeat with $v_2$, forming $J_2$, and continue until a perfect matching is found.
    \item
      This generates a random matching $\pi$ with probability
      \[\mu(\pi) = \prod_{i = 1}^n \abs{J_i}^{-1}.\]
  \end{itemize}
\end{algorithm}
% First, note that $G$ always contains the matching $\{(1, 1'), \ldots, (n, n')\}$. Consider the following sequential algorithm for sampling a random matching from $G$:
% \begin{itemize}
%   \item[1.]
%     In the order $i = 1, 2, \ldots, t_1$, match $i$ uniformly at random to an unmatched $j'$, with $(i, j') \in E$.
%   \item[2.]
%     For $i = t_1 + 1, t_1 + 2, \ldots, n$, match $i$ to $(i - t_1)'$ if $(i - t_1)'$ is unmatched. Otherwise, match $i$ uniformly at random to an unmatched $j'$, with $(i, j') \in E$.
% \end{itemize}
Importance sampling can then be used to estimate $M(G) = \abs{\mc{M}(G)}$ using the estimator
\[\hat{M}(G) = \frac{1}{N} \sum_{i = 1}^N \frac{1}{\mu(\pi_i)},\]
where $\pi_1, \ldots, \pi_N$ are i.i.d.\ samples from $\mu$. \\
$\mu$ takes a particularly simple form when $G$ is the bipartite graph given by the type-$(s, t)$ restriction matrix.
% Diaconis and Kolesnik~\cite{dk19} analyze both the \emph{top-down} algorithm, where $(v_1, \ldots, v_n) = (1, 2, \ldots, n)$, and the \emph{random-order} algorithm, where $(v_1, \ldots, v_n)$ is a random permutation of $[n]$, for $t$-Fibonacci and distance-2 permutations. This work analyzes the top-down algorithm for general type-$(s, t)$ permutations $\mc{F}_{n, s, t}$.
% TODO: maybe summarize Diaconis/Kolesnik?
\begin{proposition}
  Let $G$ be a type-$(t_1, t_2)$ bipartite graph, and let $v_i = i$ in Algorithm~\ref{alg:sequential}. Then,
  \[\abs{J_i} \in \{1, \min(t_2 + 1, n - i + 1)\}.\]
\end{proposition}
\begin{proof}
  The following properties hold at step $i$ of the algorithm.
  \begin{itemize}
    \item[1.]
      The vertices $1', 2', \ldots, (i - t_1 - 1)'$ have all been matched.
    \item[2.]
      Exactly $i - 1$ vertices in $[\min((i + t_2)', n')]$ have been matched.
  \end{itemize}
  If $(i - t_1)'$ is unmatched at step $i$, then $J_i = \{(i - t_1)'\}$. Otherwise, $J_i$ contains exactly $\min(i + t_2, n) - (i - 1) = \min(t_2 + 1, n - i + 1)$ vertices.
\end{proof}
It follows that
\begin{equation}\label{eq:sampling_distribution}
  \mu(\pi) = C(\pi)^{-1} \cdot (t_2 + 1)^{-s(\pi)},
\end{equation}
where $s(\pi) = \#\{i \le n - t_2: \abs{J_i} \ne 1\}$. The coefficient $C(\pi)^{-1}$ is the contribution from $\{J_i: n - t_2 < i \le n\}$ and is bounded below by $(t_2!)^{-1}$.
% One need not sample $\pi(i)$ in the order $i = 1, 2, \ldots, n$. Instead, one can consider first choosing $i$ uniformly among vertices that have not yet been matched, and then choosing $\pi(i)$ uniformly at random from all choices of $\pi(i)$ such that the resulting semi-matching can be completed to a perfect matching. This is known as the randomized sampling algorithm in~\cite{dk19}. Finally, for type-$(t, 1)$ permutations, there exists an ordering $i_1 \ne i_2 \ne \cdots \ne i_n$ such that the KL divergence between $\mu$ and uniformity is minimized. For example, for Fibonacci permutations, we first sample $\pi(i)$ for $i = 2, 5, 8, \ldots, 3k - 1$, where $k$ is the largest integer such that $3k - 1 \le n$.
% What remains is to characterize the distribution of the number of times the algorithm is forced to make a certain choice ($\abs{C_i} = 1$). In the plots in the next section, one can see that it is approximately normal. We now outline the difficulties in one approach (Stein's method) to proving normality. \\
% Let $f: S(A) \rightarrow \Z$ denote the number of times the algorithm is forced to make a choice for a given permutation. Stein's method requires us to construct an exchangeable pair $W, W' \in S(A)$, such that $f(W)$ and $f(W')$ are close. More precisely,~\cite{cha14} tells us that we need some small $\lambda$ such that
% \begin{align*}
%   \E(f(W') - f(W) \mid W) &= -\lambda W + o(\lambda) \\
%   \E[(f(W') - f(W))^2 \mid W] &= 2\lambda + o(\lambda) \\
%   \E \abs{f(W') - f(W)}^3 &= o(\lambda).
% \end{align*}
% Typically, the exchangeable pair is obtained by taking one step in a Markov chain that has $W$ as its stationary distribution. This suggests that taking $W'$ to be $W$ composed with a random transposition does not work, since the number of possible transpositions is $O(n)$, while the permutations with the largest and smallest probabilities differ by a factor that is exponential in $n$. \\
% Another idea is to construct $W'$ by resampling a particular step in the algorithm. However, since all steps are history-dependent, there is little reason to expect $f(W)$ and $f(W')$ to be close. \\
% For a permutation $\pi \in S_n$, the sets $b_1(\pi), \ldots, b_m(\pi)$ form a \emph{block decomposition of} $\pi$ if the following conditions hold:
% \begin{itemize}
%   \item[1.]
%     $b_1(\pi) \cup b_2(\pi) \cup \cdots \cup b_m(\pi) = [n]$
%   \item[2.]
%     There exist integers $i_1 < i_2 < \cdots < i_{k - 1}$ such that all elements in $b_j$ are between $i_{j - 1} + 1$ and $i_j$
%   \item[3.]
%     If $\pi(a) = b$, then both $a$ and $b$ are elements of the same block
% \end{itemize}
% Define the \emph{maximal block decomposition} of $\pi$ as the block decomposition $\bar{b} = (b_1(\pi), \ldots, b_m(\pi))$ where $m$ is maximized. \\
% Conditional on the block decomposition $\bar{b}$, the permutations within each block are mutually independent. Thus, the number of times the algorithm has a single choice is a sum over $T$ independent random variables, where $T$ is the length of the maximal block decomposition.
% Let us examine what a permutation $\pi \in S(A)$ looks like. We note that cycles can have arbitrary length, and that any cycle $(a_1, a_2, \ldots, a_m)$ of length $m \ge 3$ must be such that $\{a_1, a_2, \ldots, a_m\} = \{i, i + 1, \ldots, j\}$, where $j - i + 1 = m$. Now, any permutation $\pi$ splits into blocks $b_1(\pi), b_2(\pi), \ldots, b_l(\pi)$, where $\pi$ does not send any element from $b_i(\pi)$ to $b_j(\pi)$ if $i \ne j$. There exists a \emph{maximal block arrangement} of $\pi$


==> clt.tex <==
% chktex-file 3
% For small values of $t$, $c_1$ and $c_2$ have the following values.
% \begin{table}[h]
%   \begin{tabular}{c|c|c}
%     t  & c_1 & c_2 \\ \hline
%     1  & 0.47640 \ldots & 0.08944 \ldots \\
%     2  & 0.44305 \ldots & 0.05950 \ldots \\
%     3  & 0.45690 \ldots & 0.03138 \ldots \\
%     4  & 0.47193 \ldots & 0.01580 \ldots \\
%     5  & 0.48270 \ldots & 0.00788 \ldots \\
%     10 & 0.49890 \ldots & 0.00024 \ldots
%   \end{tabular}
% \end{table}
This section focuses on
\subsection{Time-inhomogeneous Markov chains}
A key observation for the analysis of Algorithm 1 is that a matching drawn uniformly from our restriction matrix is representable by a time-inhomogeneous markov chain $X_0, X_1, \ldots, X_n$ with a fixed starting state. Central limit theorems for these chains were first studied by Dobrushin~\cite{dob56}. Sethuraman et.\ al.\ later gave a shorter proof using martingale techniques~\ref{sv05}. Both proofs set conditions on the contraction coefficient
\[\delta(\pi) = \sup_{\substack{x_1, x_2 \\ u \in \mc{U}}} \abs{(\pi u)(x_1) - (\pi u)(x_2)}.\]
Peligrad~\cite{pel12} later modified Dobrushin's theorem into one that imposes a condition on the maximal correlation coefficient
\begin{align*}
  \rho(A, B) &= \sup_{\substack{\E f = \E g = 0 \\ \E f^2 = \E g^2 = 1}} \abs{\corr{f(A), g(B)}} \\
  \rho_n &= \max_{1 \le s \le n} \rho(X_{s - 1}, X_s).
\end{align*}
We use the following central limit theorem, as it apperas in~\cite{pel12}.
\begin{theorem}\label{thm:TIMC_clt}
  Let $X_{n, 1}, \ldots, X_{n, n} \in \mc{X}$ be a time-inhomogeneous Markov chain. Define the maximal correlation coefficient $\rho_n$ as above. \\
  Let $\lambda_n = 1 - \rho_n$, and let $Y_{n, i} = f_{n, i}(X_{n, i})$, where $(f_{n, i})_{1 \le i \le n}$ are real-valued functions on $\mc{X}$. Denote by $\mu_n$ and $\sigma^2_n$, respectively, the mean and variance of $\sum_{i = 1}^n Y_{n, i}$. Suppose
  \[\max_{1 \le i \le n} \abs{Y_{n, i}} \le C_n \text{~a.s.}\]
  and
  \[\frac{C_n(1 + \abs{\ln(\lambda_n)})}{\lambda_n \sigma_n} \rightarrow 0 \text{~as~} n \rightarrow \infty.\]
  Then
  \[\frac{\sum_{i = 1}^n Y_{n, i} - \mu_n}{\sigma_n} \overset{d}\rightarrow N(0, 1).\]
\end{theorem}
A sufficient condition for the central limit is implied, for instance, by
\[(1 - \rho_n)^3 n (\ln n)^{-2} \rightarrow \infty \text{~as~} n \rightarrow \infty.\]
If $K$ is a transition matrix
For type-$(t_1, t_2)$ permutations, it turns out that $1 - \rho_n > \epsilon$, where $\epsilon$ depends only on $t_1$ and $t_2$.
The remainder of this section will be devoted to bounding $\rho_n$ for type-$(t_1, t_2)$ permutations.
The proof of Theorem~\ref{thm:IS_clt} uses a central limit theorem for inhomogeneous Markov chains established in~\cite{pel12}.
To use Theorem~\ref{thm:TIMC_clt}, one must show that $\lambda_n$ doesn't decay to 0 too quickly. For $t$-Fibonacci sequences, we prove the stronger result that $\rho_n$ is bounded away from 1 by a constant that is independent of $n$. The proof of this uses the following proposition.
\begin{proposition}\label{prop:max_corr}
  Let $\Omega$ be a finite state space, and let $X, Y$ be two random variables on $\Omega \times \Omega$ with joint law $\mu(x, y)$. Let $\mc{H}$ be the graph with vertex set $\Omega$ and edge set $E = \{(x, y): \mu(x, y) > 0\}$. Then, if $\rho(X, Y) = 1$, then $\mc{H}$ is either bipartite or disconnected.
\end{proposition}
\begin{proof}
  Suppose $f, g: \Omega \rightarrow \R$ are functions such that $\E f = \E g = 0$, $\E f^2 = \E g^2 = 1$, and $\text{corr}(f(X), g(Y)) = 1$. Then, there exist $a > 0, b$ such that $g(y) = af(x) + b$ for all $(x, y) \in E$. Let $c$ be some value in the range of $f$, and define
  \begin{align*}
    S &= \{x \in \Omega: f(x) = c\} \\
    T &= \{y \in \Omega: g(y) = ac + b\}.
  \end{align*}
  Since $f$ and $g$ are both nonconstant, $S$ and $T$ are both strict subsets of $\Omega$. Moreover, $T = \mc{N}(S)$ and $T^c = \mc{N}(S^c)$, where $\mc{N}(S)$ denotes the neighborhood of $S$. \\
  Let $R_1 = T \cap S^c$ and $R_2 = T^c \cap S$. Then, $S \backslash R_2$ and $S^c \backslash R_1$ are components disconnected from the rest of $\mc{H}$. If $R_2 = S$ and $R_1 = S^c$, then $\mc{H}$ is bipartite. This completes the proof.
\end{proof}
\begin{proof}[Proof of Theorem~\ref{thm:IS_clt}]
  The state graph $\mc{H}$ is clearly connected, and since $0$ connects to itself, $\mc{H}$ is not bipartite. Thus, $\rho_n < 1$ by Proposition~\ref{prop:max_corr}.
  Next, the transition matrices $K_i(x, y)$ have entries that are bounded by
  \[\varphi_t \le K_i(x, y) \le 1 - \varphi_t,\]
  where $\varphi_t$ is a constant independent of $n$. Thus, there exists a $c_t > 0$ that is independent of $n$ such that $\rho_n \le 1 - c_t$. \\
  This bound on $\rho_n$ is sufficient for Theorem~\ref{thm:TIMC_clt}.
\end{proof}
% \begin{theorem}\label{thm:cycle_clt}
%   Let $N(m)$ be defined as above. Then
%   \[P\left( \frac{N(m) - \E N(m)}{\sqrt{\Var N(m)}} < t \right) \underset{m \rightarrow \infty}\rightarrow \frac{1}{\sqrt{2\pi}} \int_{-\infty}^t e^{-\frac{t^2}{2}} dt\]
% \end{theorem}
% \begin{proof}
%   Let $p_1, p_2, \ldots, p_t$ be defined by the equations~\eqref{eq:opt_sampling_probs}, and let $X_1, X_2, \ldots$ be iid with the following distribution: for $1 \le k \le t$, $P(X_1 = k) = (1 - p_k)\prod_{i = 1}^{k - 1} p_i$, and $P(X_1 = t + 1) = 1 - \sum_{i = 1}^t P(X_1 = t)$. Let $S_n = \sum_{i = 1}^n X_i$, and let $T_N = \inf\left\{ n: S_n > N \right\}$. Note that $\{S_n\}_{n \ge 0}$ forms a renewal process. By the renewal theorem, we have $\frac{T_N}{N} \rightarrow \frac{1}{\mu}$ in probability, and that the counting process $T_N$ satisfies the limit theorem
%   \[\frac{T_N - \mu}{\sigma^2} \rightarrow N(0, 1),\]
%   where $\sigma^2 = \Var N \cdot \sqrt{N/\mu^3}$. \\
%   Consider a map $\varphi$ between the sequence $X_1, X_2, \ldots$ and type-$(t, 1)$ permutations on $1, 2, \ldots, m$ defined as follows: $\pi(X_1, \ldots, X_{T_m - 1})$ is obtained by composing the cycles $(S_{i - 1} + 1, \ldots, S_i)$ for each $1 \le i \le T_m - 1$ as well as the cycle $(S_{T_m - 1} + 1, \ldots, m)$. It is clear that the first $S_{T_m - 1}$ elements in $\pi(X_1, \ldots, X_{T_m - 1})$ is distributed according to the sampling model with probabilities $p_1, \ldots, p_t$. Since sampling using $p_1, \ldots, p_t$ gives us a uniformly distributed type-$(t, 1)$ permutation, we have $N(T_m - 1) \overset{d}= \#\{k \le T_m - 1: X_k = t + 1\}$. Finally, we note that proving the asymptotic normality of $\lim_{m \rightarrow \infty} N(T_m - 1)$ also gives the same result for $\lim_{m \rightarrow \infty} N(T_m)$ and $\lim_{m \rightarrow \infty} N(m)$, since $N(m), N(T_m),$ and $N(T_m - 1)$ all differ by at most 1. \\
%   Now, recall Anscombe's Theorem for the sum of a random number of iid random variables:
%   \begin{theorem}[Anscombe]
%     Let $\{Y_k, k \ge 1\}$ be a sequence of iid random variables with mean 0 and finite variance $\sigma^2$, and let $\{S_n, n \ge 1\}$ denote their partial sums. Let $M(n)$ be random variables such that
%     \[\frac{M(n)}{n} \overset{p}\rightarrow \theta\]
%     for some $0 < \theta < \infty$. Then
%     \begin{itemize}
%       \item[(i)]
%         \[\frac{S_{M(n)}}{\sigma \sqrt{M(n)}} \overset{d}\rightarrow N(0, 1) \qquad \text{as~} t \rightarrow \infty\]
%       \item[(ii)]
%         \[\frac{S_{M(n)}}{\sigma \sqrt{n \theta}} \overset{d}\rightarrow N(0, 1) \qquad \text{as~} t \rightarrow \infty\]
%     \end{itemize}
%   \end{theorem}
%   In our exercise, $M(n) = T_n$, $Y_i = \I\{X_i = t + 1\}$, and $\theta = \frac{1}{\mu}$. Anscombe's theorem therefore gives us
%   \[\frac{N(T_n) - P(X_1 = t + 1)T_n}{\sigma \sqrt{n/\mu}} = \frac{\sum_{i = 1}^{T_n} \I\{X_i = t + 1\} - P(X_1 = t + 1) T_n}{\sigma \sqrt{n\theta}} \underset{n \rightarrow \infty}\rightarrow N(0, 1).\]
%   Since $T_n$ itself converges to a normal distribution, we get that asymptotically, $N(T_n)$ is a linear combination of Gaussians and is therefore also Gaussian. This concludes the proof.
% \end{proof}
% As a remark, note that there is nothing special about the statistic $T_n = \#\{i: \pi(i) = i - t\}$. Theorem~\ref{thm:cycle_clt} very easily extends to other statistics of restricted permutations one might be interested in.
\subsubsection{Comparison to Variance Estimator}
Suppose we want to count the number of perfect matchings in a $t$-Fibonacci graph by importance sampling. Let $N$ be the minimum number of samples such that
Under the naive sampling algorithm, we have $p_1 = p_2 = \cdots = p_t = 1/2$. Thus,
\[\log \frac{d\nu}{d\mu}(\pi) = -\log F_{n + 1}^{(t)} + (n - 1 - k(\pi)) \log 2.\]
The variance is therefore
\[\Var\left( \log \frac{d\nu}{d\mu} \right) = (\log 2)^2 \Var s(\pi).\]
In the na\"{i}ve variance bound, we require that
\begin{align*}
  N &\simeq \frac{\Var 1/p(\pi)}{(\E 1/p(\pi))^2} \\
  &= \frac{\Var 2^{n - 1 - k(\pi)}}{(F_{n+1}^{(t)})^2} \\
  &= \frac{2^{2n - 2}}{(F_{n+1}^{(t)})^2} \Var(2^{-k(\pi)})
\end{align*}
Observe that $2^{-k(\pi)} = \exp(-k(\pi) \log 2)$ is asymptotically a log-normal distribution with variance
\begin{align*}
  \Var(2^{-k(\pi)}) &= (e^{(\log 2)^2 \Var(k(\pi))} - 1)(e^{-2 \log 2 \E k(\pi) + (\log 2)^2 \Var(k(\pi))}) \\
  &= (e^{(\log 2)^2 (c_2 n + O(1))} - 1)(e^{(-2c_1 \log 2 + c_2(\log 2)^2)n + O(1)}) \\
  &\simeq e^{(-2c_1 \log 2 + 2c_2 (\log 2)^2)n}
\end{align*}
Observe that in the variance bound, the required sample size takes the form $N_{req} = C_1 e^{C_2 n}$, where $C_1$ and $C_2$ are constants independent of $n$. Constrasting this to the $e^L$ estimator, where a sample size of $e^{L + O(\sqrt{n})}$ is required, it is clear that the $e^L$ estimator is asymptotically much better.
\subsection{Generalizations}
The Markov chain approach can be generalized to type-$(t_1, t_2)$ permutations by expanding the state space.
\begin{proposition}
  Let $t_1, t_2 > 0$, and let $G = ([n], [n'], E)$, where $(i, j') \in E$ if and only if $-t_1 \le j - i \le t_2$. Let $M$ be a matching drawn uniformly at random from the set of perfect matchings on $G$, and $E_i \in [n']$ be the set of unmatched vertices adjacent to $v_i = i$ when sampling $M$ using Algorithm 1. Let $X_i = E_i - i = \{e - i: e \in E_i\}$. Then, $\{X_i\}_{i = 1}^n$ is a time-inhomogeneous Markov chain on the state space $\mc{X} = \{-t_1, -t_1 + 1, \ldots, t_2\}$ with initial state $X_1 = \{0, 1, \ldots, t_2\}$ and transition probabilities
  \[P(X_{i + 1} = \{t_2'\} \cup (X_i \backslash x - 1') \mid X_i = x_i) = \begin{cases}
    1 &\mbox{if~} -t_1' \in x_i \text{~and~} x = -t_1' \\
    \frac{M(x, x_i)}{\sum_{y \in x_i}M(y, x_i)} &\mbox{if~} -t_1' \not\in x_i \text{~and~} x \in x_i \\
    0 &\mbox{otherwise}
  \end{cases}\]
  where $M(x, x_i)$ is the number of perfect matchings in the graph $G(x, x_i) = (U_i, V(x, x_i), E(x, x_i))$, where $U_i = \{i + 1, \ldots, n\}$, $V(x, x_i) = (x_i \backslash x + i') \cup \{(i + 3)', \ldots, n'\}$, and $E(x, x_i)$ is the restriction of $E$ onto the subgraph defined by the vertices $U_i$ and $V(x, x_i)$.
  % Let $Y_i = X_i + i$ for all $i$, and let $G = ([n], [n'], E)$, where $(i, j') \in E$ if and only if $-t_1 \le i - j \le t_2$. Let $M$ be the matching sampled using Algorithm 1 in the order $(v_1, \ldots, v_n) = (1, 2, \ldots, n)$ with $J_i = Y_i$ at step $i$. Then $M$ is uniformly distributed on perfect matchings of $G$.
\end{proposition}
\begin{proof}
  % In the order $i = 1, 2, \ldots, n$, construct $M$ by matching $i$ to $(i + a_{i, k})'$ for the transition $X_i \rightarrow \{t_2\} \cup (X_i \backslash a_{i, k} - 1)$. \\
  Suppose it is given that $X_1 = x_1, \ldots, X_i = x_i$ for some $x_1, \ldots, x_i \in \{-t_1', \ldots, t_2'\}^{t_2 + 1}$. If $-t_1' \in x_i$, then $(i - t_1)'$ is not matched to any of the vertices $1, 2, \ldots, i - 1$. Thus, the only semimatching that is extendable to a perfect matching connects $i$ with $(i - t_1)'$. Therefore in this case,
  \begin{align*}
    &P(X_{i + 1} = \{t_2\} \cup (X_i \backslash \{-t_1\} - 1) \mid X_1 = x_1, \ldots, X_i = x_i)  \\
    &\qquad= P(X_{i + 1} = \{t_2\} \cup (X_i \backslash \{-t_1\} - 1) \mid X_i = x_i) = 1
  \end{align*}
  On the other hand, if $-t_1' \not\in x_i$, then any choice of $x$ is extendable to a perfect matching. For $M$ to be uniformly distributed, the probability of the transition $X_i \rightarrow \{t_2'\} \cup (X_i \backslash x - 1')$ must be proportional to the number of perfect matchings of $G(x, x_i)$. In particular, this probability is independent of $X_1, \ldots, X_{i - 1}$ and is precisely $\frac{M(x, x_i)}{\sum_{y \in x_i}M(y, x_i)}$.
\end{proof}
In the sequential importance sampling algorithm, a move is forced at each state which contains $-t_1$. The required sample size to form an accurate estimate on the number of matchings requires a tail bound the number of such states $s(\pi)$. As with $t$-Fibonacci sequences, we prove a central limit theorem for the quantity $\sum_{i = 1}^n \I(-t_1 \in X_i)$.
\begin{theorem}\label{thm:IS_clt_general}
  Let $s(\pi)$ be defined as above. Then,
  \[\frac{s(\pi) - \E_\nu s(\pi)}{\sqrt{\Var_\nu(s(\pi))}} \overset{d}\rightarrow N(0, 1).\]
  It therefore follows that $e^{L + c\sqrt{n}}$ samples suffice for importance sampling, for some constant $c$.
\end{theorem}
\begin{proof}
  Recall that transitions between states are of the form
  \[(a_1, a_2, \ldots, a_{t_2}, a_{t_2 + 1} = t_2) \rightarrow (a_1 - 1, a_2 - 1, \ldots, a_{i - 1} - 1, a_{i + 1} - 1, \ldots, a_{t_2} - 1, a_{t_2 + 1} - 1, t_2).\]
  Call the transition where $a_i$ is removed $T_i$. \\
  State $(0, 1, 2, \ldots, t_2)$ connects to state $(a_1, a_2, \ldots, a_{t_2}, t_2)$ by applying the transition $T_{i + 1}$ $a_{i + 1} - a_i$ times, for each $i = 1, 2, \ldots, t_2$. This shows that $\mc{H}$ is connected. Next, observe that the state $(0, 1, 2, \ldots, t_2)$ connects to itself by applying $T_1$, so $\mc{H}$ is not bipartite. Thus, by Proposition~\ref{prop:max_corr}, $\rho_n < 1$. \\
  Next, note that there exists a constant $\varphi_t > 1$, independent of $n$, such that
  \[\varphi_t^{-t} \le \frac{M(x, x_i)}{\sum_{y \in x_i} M(y, x_i)} \le 1 - \varphi_t^{-t}.\]
  So the transition probabilities are either 1 or bounded away from $\{0, 1\}$ by a constant that is independent of $n$. Thus, $\rho_n \le 1 - c_t$, where $c_t$ is independent of $n$. This means that Theorem~\ref{thm:TIMC_clt} is applicable, and the desired central limit theorem follows.
\end{proof}
% We now turn to the general case of restrictions with perfect sampling probabilities. To that end, we have the following result:
% \begin{theorem}
%   Suppose the restriction $A$ admits a set of perfect sampling probabilities. Let $A_n$ be the restriction matrix formed by taking the first $n$ rows and columns of $A$. For a restricted permutation $\pi$ and fixed $j > 0$, define the statistic $T = \#\{i: \pi(i) = i + j\}$. Then,
%   \[\frac{T - \E T}{\sqrt{\Var T}} \overset{d}\rightarrow N(0, 1).\]
% \end{theorem}
% Thus, the performance of an estimator is determined by the exponential rate $C_2$. Using the formulas provided by Diaconis/Fan/Graham, we get the following table of values for the $e^L$ estimator and the na\"{i}ve variance bound:
% \begin{table}[h]
%   \begin{tabular}{c|c|c}
%     t & e^L & Variance \\ \hline
%     1  & 0.08944 & 0.12665 \\
%     2  & 0.0595  & 0.08693 \\
%     3  & 0.03138 & 0.04707 \\
%     4  & 0.0158  & 0.02414 \\
%     5  & 0.00788 & 0.01218 \\
%     6  & 0.00393 & 0.00612 \\
%     7  & 0.00196 & 0.00307 \\
%     8  & 0.00098 & 0.00153 \\
%     9  & 0.00049 & 0.00077 \\
%     10 & 0.00024 & 0.00038
%   \end{tabular}
% \end{table}
% \subsubsection{Use in Importance Sampling}
% Recall that our original sampling algorithm for generating a random type-$(t, 1)$ permutation had $p_1 = p_2 = \cdots = p_t = \frac{1}{2}$. In that case, the KL divergence $L$ between the sampling distribution $\nu$ and the uniform distribution $\mu$ is given by
% \begin{align*}
%   L = D_{KL}(\mu \| \nu) &= \E_\mu\left( \log \frac{d\mu}{d\nu} \right) \\
%   &= \E_\mu\left( (n - 1 - f(\pi)) \log 2 - \log F_{n + 1}^{(t)} \right),
% \end{align*}
% where $f(\pi)$ denotes the number of $(t + 1)$-cycles of $\pi$. Since we have just shown that $f(\pi)$ has a limiting normal distribution, it follows that $L$ also has a limiting normal distribution. Thus, the bound provided by Chatterjee/Diaconis blahblah


==> generating_functions.tex <==
% chktex-file 3
% \subsection{Summary}
% \begin{itemize}
%   \item
%     For permutations of type $(t, 1)$, with $t \ge 1$, the generating function $G(z, x) = \sum_{n = 0}^\infty z^n \sum_{\pi \in S_{n t}} x^{k(\pi)}$ has the closed form
%     \[G(z, x) = \frac{P(z, x)}{Q(z, x)} = \frac{1 + z(1 - x)\sum_{i = 0}^{t - 1} x^i z^i}{1 - xz - x^2 z^2 - \cdots - x^t z^t - x^t z^{t + 1}}.\]
%   \item
%     For any $x \ge 1$, $Q(z, x)$ has a unique positive real root $r$, which also happens to be the root of smallest norm.
%   \item
%     We may write $G(z, x)$ as
%     \[G(z, x) = \sum_i \left( \frac{a_{i1}}{z - r_i} + \frac{a_{i2}}{(z - r_i)^2} + \cdots + \frac{a_{i k_i}}{(z - r_i)^{k_i}} \right),\]
%     where $k_i$ is the multiplicity of the root $r_i$. Since $r$ is a simple root, the coefficient corresponding to $\frac{1}{z - r}$ is
%     \[\frac{P(x, z)}{Q'(x, z)} = -\frac{1 + z(1 - x)\sum_{i = 0}^{t - 1} x^i z^i}{x(1 + 2xz + 3x^2 z^2 + \cdots + t x^{t - 1} z^{t - 1} + (t + 1) x^{t - 1}z^t)}.\]
%   \item
%     For small values of $t$ and $t \rightarrow \infty$, we can compute the following table: \\
%     % \begin{table}[h]
%     %   \begin{tabular}{c|c|c|c|c|c}
%     %     t & r_1 & c_1 & r_2 & c_2 & (\log N) / n \\ \hline
%     %     1  & 0.61803 & 0.723606 & 0.36602 & 0.50000 & 0.04262 \\
%     %     2  & 0.54368 & 0.618419 & 0.28737 & 0.36012 & 0.02822 \\
%     %     3  & 0.51879 & 0.566342 & 0.26512 & 0.30612 & 0.01505 \\
%     %     4  & 0.50866 & 0.537926 & 0.25675 & 0.28047 & 0.00768 \\
%     %     5  & 0.50413 & 0.521772 & 0.25317 & 0.26699 & 0.00387 \\
%     %     6  & 0.50201 & 0.512454 & 0.25153 & 0.25955 & 0.00194 \\
%     %     7  & 0.50099 & 0.507071 & 0.25075 & 0.25537 & 0.00097 \\
%     %     8  & 0.50049 & 0.503980 & 0.25037 & 0.25300 & 0.00048 \\
%     %     9  & 0.50024 & 0.502220 & 0.25018 & 0.25167 & 0.00024 \\
%     %     10 & 0.50012 & 0.501227 & 0.25009 & 0.25092 & 0.00012 \\
%     %     11 & 0.50006 & 0.500673 & 0.25004 & 0.25050 & 6.10105 \cdot 10^{-5} \\
%     %     12 & 0.50003 & 0.500366 & 0.25002 & 0.25027 & 3.05105 \cdot 10^{-5} \\
%     %     13 & 0.50001 & 0.500198 & 0.25001 & 0.25014 & 1.52567 \cdot 10^{-5} \\
%     %     14 & 0.50000 & 0.500106 & 0.25000 & 0.25008 & 7.62883 \cdot 10^{-6} \\
%     %     15 & 0.50000 & 0.500057 & 0.25000 & 0.25004 & 3.81454 \cdot 10^{-6} \\
%     %     16 & 0.50000 & 0.500030 & 0.25000 & 0.25002 & 1.90730 \cdot 10^{-6} \\
%     %     17 & 0.50000 & 0.500016 & 0.25000 & 0.25001 & 9.53662 \cdot 10^{-7} \\
%     %     18 & 0.50000 & 0.500008 & 0.25000 & 0.25000 & 4.76834 \cdot 10^{-7} \\
%     %     19 & 0.50000 & 0.500004 & 0.25000 & 0.25000 & 2.38417 \cdot 10^{-7} \\
%     %     \infty & 0.5 & 0.5 & 0.25 & 0.25 & 0
%     %   \end{tabular}
%     % \end{table} \\
%     The asymptotics of $\E T$ and $\Var T$ (as $n \rightarrow \infty$) are equal to $c_1 r_1^{-n}$ and $c_2 r_2^{-n} - c_1^2 r_1^{-2n}$, respectively.
%   \item
%     The KL divergence between the sampling distribution and the uniform distribution is given by
%     \[D_{KL}(\mu \| \nu) = \E_\mu(\log d\nu/d\mu) \propto \sum_\pi k(\pi).\]
%     Letting $g_n(k)$ be the number of restricted permutations with $k(\pi) = k$, we get that
%     \begin{align*}
%       \sum_\pi k(\pi) &= \sum_{0 \le k \le n - 1} g_n(k) \\
%       &= \frac{\partial}{\partial x} G(x, z) \biggr|_{x = 1}[z^n],
%     \end{align*}
%     where $f(z)[z^n]$ denotes the coefficient of $z^n$ in the power series expansion of $f(z)$. We have
%     \[\frac{\partial}{\partial x} G(x, z) \biggr|_{x = 1} = \frac{z^2 \sum_{i = 0}^{t - 1} (i + 1) z^i}{1 - z - \cdots - z^{t + 1}} + \frac{z^2 \sum_{i = 0}^t z_i (1 + 2z + \cdots + tz^{t - 1} + tz^t)}{(1 - z - \cdots - z^{t + 1})^2}.\]
%     The second term determines the asymptotic behavior of this rational function.
% \end{itemize}
% \[\begin{pmatrix}
%   1 & 1 & \cdots & 1 & 0 & 0 & \cdots & 0 \\
%   1 & 1 & \cdots & 1 & 1 & 0 & \cdots & 0 \\
%   \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
%   1 & 1 & \cdots & & & & & \\
%   0 & 1 & \cdots & & & & & \\
%   \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
%   0 & 0 & \cdots & & & & &
% \end{pmatrix}\]
% \begin{example}[$s = t = 2$]
%   The states in type-$(2, 2)$ sequences are the pairs
%   \[\{(0, 1), (-1, 1), (-1, 0), (-2, 1), (-2, 0), (-2, -1)\}.\]
%   Here, the recurrence relations are
%   \begin{align*}
%     [0, 1]^n_m &= 3^m([0, 1]^{n - 1}_m + [-1, 1]^{n - 1}_m + [-1, 0]^{n - 1}_m) \\
%     [-1, 1]^n_m &= 3^m([0, 1]^{n - 1}_m + [-2, 1]^{n - 1}_m + [-2, 0]^{n - 1}_m) \\
%     [-1, 0]^n_m &= 3^m([-1, 1]^{n - 1}_m + [-2, 1]^{n - 1}_m + (-2, -1)^{n - 1}_m) \\
%     [-2, 1]^n_m &= [0, 1]^{n - 1}_m \\
%     [-2, 0]^n_m &= [-1, 1]^{n - 1}_m \\
%     [-2, -1]^n_m &= [-2, 1]^{n - 1}_m = [0, 1]^{n - 2}_m.
%   \end{align*}
%   Further simplification yields
%   \begin{align*}
%     [0, 1]^n_m &= 3^m([0, 1]^{n - 1}_m + [-1, 1]^{n - 1}_m) + 3^{2m}([-1, 1]^{n - 2}_m + [0, 1]^{n - 3}_m + [0, 1]^{n - 4}_m) \\
%     [-1, 1]^n_m &= 3^m([0, 1]^{n - 1}_m + [0, 1]^{n - 2}_m + [-1, 1]^{n - 2}_m).
%   \end{align*}
%   The generating functions $X(z, m)$ and $X'(z, m)$, defined by
%   \begin{align*}
%     X = X(z, m) &= \sum_{n = 0}^\infty [0, 1]^n_m z^n \\
%     X' = X'(z, m) &= \sum_{n = 0}^\infty [-1, 1]^n_m z^n
%   \end{align*}
%   with the partial sums
%   \begin{align*}
%     X_k = X_k(z, m) &= \sum_{n = 0}^k [0, 1]^n_m z^n \\
%     X'_k = X'_k(z, m) &= \sum_{n = 0}^k [-1, 1]^n_m z^n
%   \end{align*}
%   are therefore given by
%   \begin{align*}
%     X &= X_3 + \sum_{n = 4}^\infty \left( 3^m([0, 1]^{n - 1}_m + [-1, 1]^{n - 1}_m) + 3^{2m}([-1, 1]^{n - 2}_m + [0, 1]^{n - 3}_m + [0, 1]^{n - 4}_m) \right)z^n \\
%     &= X_3 + 3^{m}z(X - X_2 + X' - X'_2) + 3^{2m} \left( z^2 (X' - X'_1) + z^3 (X - 1) + z^4 X \right) \\
%     X' &= X'_1 + 3^m \sum_{n = 2}^\infty \left( [0, 1]^{n - 1}_m + [0, 1]^{n - 2}_m + [-1, 1]^{n - 2}_m \right) z^n \\
%     &= X'_1 + 3^m \left( z(X - 1) + z^2 X + z^2 X' \right).
%   \end{align*}
%
%   Solving this system yields the asymptotic results
%   \begin{align*}
%     \E_\nu \log \frac{1}{P(Y)} &= 0.9053n + O(1) \\
%     \Var_\nu \log \frac{1}{P(Y)} &= 0.1147n + O(1),
%   \end{align*}
%   Details of the computation can be found in~\cite{dk19}.
% \end{example}
  % \begin{align*}
  %   [0, 1]^n &= [0, 1]^{n - 1} + [-1, 1]^{n - 1} + [-1, 0]^{n - 1} \\
  %   [-1, 1]^n &= [0, 1]^{n - 1} + [-2, 1]^{n - 1} + [-2, 0]^{n - 1} \\
  %   [-1, 0]^n &= [-1, 1]^{n - 1} + []
  %   % [0, 1, 2]^n &= [0, 1, 2]^{n - 1} + [-1, 1, 2]^{n - 1} + [-1, 0, 2]^{n - 1} + [-1, 0, 1]^{n - 1} \\
  %   % [-1, 1, 2]^n &= [0, 1, 2]^{n - 1} + [-2, 1, 2]^{n - 1} + [-2, 0, 2]^{n - 1} + [-2, 0, 1]^{n - 1} \\
  %   % [-1, 0, 2]^n &= [-1, 1, 2]^{n - 1} + [-2, 1, 2]^{n - 1} + [-2, -1, 2]^{n - 1} + [-2, -1, 1]^{n - 1} \\
  %   % [-1, 0, 1]^n &= [-1, 0, 2]^{n - 1} + [-2, 0, 2]^{n - 1} + [-2, -1, 2]^{n - 1} + [-2, -1, 0]^{n - 1} \\
  %   % [-2, 1, 2]^n &= [0, 1, 2]^{n - 1} \\
  %   % [-2, 0, 2]^n &= [-1, 1, 2]^{n - 1} \\
  %   % [-2, 0, 1]^n &= [-1, 0, 2]^{n - 1} \\
  %   % [-2, -1, 2]^n &= [-2, 1, 2]^{n - 1} = [0, 1, 2]^{n - 2} \\
  %   % [-2, -1, 1]^n &= [-2, 0, 2]^{n - 1} = [-1, 1, 2]^{n - 2} \\
  %   % [-2, -1, 0]^n &= [-2, -1, 2]^{n - 1} = [0, 1, 2]^{n - 3}.
  % \end{align*}

% Define the generating function
% \[G_{T, s, t}(z) = \sum_{k = 0}^\infty z^k \sum_{Y \in \mc{T}_{k, s, t}} \theta(Y).\]
% For ease of notation, $T(n, t_1, t_2)$ will be shortened to $T(n, t)$ for type-$(t, 1)$ permutations. Consider the statistic
% \[T_{n, t}(x) = \sum_{\pi \in \mc{F}_{n, t}} x^{\tilde{s}(\pi)},\]
% where $\tilde{s}(\pi)$ is the number of $(t + 1)$-cycles in $\pi$ and differs from $s(\pi)$ by at most 1. \\
% The associated generating function $G_{T, t}$ is of particular interest in importance sampling since the quantity
% \[\log \rho(\pi) = (n - 1 - s(\pi)) \log 2 - \log F_{n + 1}\]
% is completely determined by $s(\pi)$.
% \begin{lemma}\label{lem:sampling_prob_closed_form}
%   $G_{T, t}$ has the closed form
%   \[G_{T, t}(z, x) = \frac{1}{1 - xz - xz^2 - \cdots - xz^t - xz^{t + 1}}\]
% \end{lemma}
% \begin{proof}
%   Let $A$ be the matrix with values
%   \[A_{ij} = \begin{cases}
%     x &\mbox{if~} j \le i \le j + t \\
%     1 &\mbox{if~} j = i + 1 \\
%     0 &\mbox{otherwise}
%   \end{cases}\]
%   For example, $A_6$ is given by
%   \[A_6 = \begin{pmatrix}
%     1 & 1 & 0 & 0 & 0 & 0 \\
%     1 & 1 & 1 & 0 & 0 & 0 \\
%     x & 1 & 1 & 1 & 0 & 0 \\
%     0 & x & 1 & 1 & 1 & 0 \\
%     0 & 0 & x & 1 & 1 & 1 \\
%     0 & 0 & 0 & x & 1 & 1
%   \end{pmatrix}\]
%   The statistic $T_{n, t}(x)$ is precisely the permanent of $A_n$. As a power series,
%   \[Per(A_n) = \sum_i C_i x^i,\]
%   where $C_i$ is the number of permutations $\pi \in \mc{F}_{n, t}$ with $\tilde{s}(\pi) = i$. \\
%   Expanding the permanent in its first row reveals that $Per(A_n)$ satisfies the recursion
%   \[Per(A_n) = Per(A_{n - 1}) + \cdots + Per(A_{n - t}) + x Per(A_{n - t - 1}).\]
%   where $Per(A_0) = Per(A_1) = \cdots = Per(A_t) = 1$. Solving the recurrence
%   \[G_{T, t}(z, x) = \sum_{n = 0}^\infty Per(A_n) z^n\]
%   gives
%   \[G_{T, t}(z, x) = \frac{1}{1 - z - z^2 - \cdots - z^t - xz^{t + 1}}.\]
% \end{proof}
\subsubsection{Asymptotics}
For fixed $n$, the first two moments of $\tilde{s}(\pi)$ with $\pi$ drawn uniformly from $\mc{F}_{n, t, 1}$ are given by the derivatives
\begin{align*}
  F_n^t \E \tilde{s}(\pi) &= \partial_x T_{n, t}(x) \biggr|_{x = 1} = [z^n] \left( \partial_x G_{T, t}(z, x) \biggr|_{x = 1} \right) \\
  F_n^t \E \tilde{s}(\pi)^2 &= \partial^2_{xx} T_{n, t}(x) \biggr|_{x = 1} + F_n^t \E \tilde{s}(\pi) = [z^n] \left( \partial^2_{xx} G_{T, t}(z, x) \biggr|_{x = 1} + F_n^t \partial_x G_{T, t}(z, x) \biggr|_{x = 1} \right).
\end{align*}
Using the closed form in Lemma~\ref{lem:sampling_prob_closed_form} gives
\begin{align*}
  \partial_x G_{T, t}(z, x) \biggr|_{x = 1} &= \frac{z^{t + 1}}{(1 - S)^2} \\
  \partial^2_{xx} G_{T, t}(z, x) \biggr|_{x = 1} &= \frac{2z^{2t + 2}}{(1 - S)^3},
\end{align*}
where $S = 1 - z - \cdots - z^{t + 1}$. \\
Now, $1 - S$ has a unique root $r \in (0, 1)$ of largest magnitude. The following approximations therefore hold for large $n$.
\begin{align}
  [z^n] \frac{S}{(1 - S)^2} &\approx [z^n] \left( \frac{c_1}{1 - z/r} + \frac{c_2}{(1 - z/r)^2} \right) \nonumber \\
  &= \left( c_1 + c_2 n \right) r^{-n} \label{eq:first_moment_approx} \\
  [z^n] \frac{2S^2}{(1 - S)^3} &\approx [z^n] \left( \frac{d_1}{1 - z/r} + \frac{d_2}{(1 - z/r)^2} + \frac{d_3}{(1 - z/r)^3} \right) \nonumber \\
  &= \left( d_1 + d_2n + \frac{d_3 n(n+1)}{2} \right) r^{-n} \label{eq:second_moment_approx}
\end{align}
where $c_1, c_2, d_1, d_2$, and $d_3$ are coefficients given by the formulas
\begin{align*}
  c_i &= \frac{1}{(-r)^i (2 - i)!} \lim_{z \rightarrow r} \frac{d^{2 - i}}{dz^{2 - i}} \left( (z - r)^2 \partial_x G_{T, t}(z, x) \biggr|_{x = 1} \right) \\
  d_i &= \frac{1}{(-r)^i (3 - i)!} \lim_{z \rightarrow r} \frac{d^{3 - i}}{dz^{3 - i}} \left( (z - r)^3 \partial^2_{xx} G_{T, t}(z, x) \biggr|_{x = 1} \right).
\end{align*}
Generally, if $f(z) = \frac{P(z)}{Q(z)}$ and $Q(z) = (z - r)^k R(z)$, where $P, Q$, and $R$ are polynomials such that $R(r) \ne 0$, then
\begin{align*}
  \frac{d}{dz} \left( (z - r)^k f(z) \right) &= \left( \frac{P'}{R} - \frac{PR'}{R^2} \right) \biggr|_{z = r} \\
  \frac{d^2}{dz^2} \left( (z - r)^k f(z) \right) &= \left( \frac{P''}{R} - \frac{PR''}{R^2} - \frac{2P' R'}{R^2} + \frac{2P(R')^2}{R^4} \right) \biggr|_{z = r}.
\end{align*}
For $\partial_x G_{T, t}(z, x) \biggr|_{x = 1}$, $P(z) = S$ and $Q(z) = (1 - S)^2$, yielding coefficients given by Table~\ref{tab:first_moment}.
% \begin{table}[h]
%   \centering
%   \begin{tabular}{c|c|c|c}
%     $t$ & $r$ & $c_1$ & $c_2$ \\ \hline
%     1 & 0.61803 & -0.43416 & 0.52361 \\
%     2 & 0.54369 & -0.25053 & 0.38244 \\
%     3 & 0.51879 & -0.15848 & 0.32074 \\
%     4 & 0.50866 & -0.10341 & 0.28936 \\
%     5 & 0.50414 & -0.06777 & 0.27225 \\
%     6 & 0.50202 & -0.04403 & 0.26261 \\
%     7 & 0.50099 & -0.02818 & 0.25712 \\
%     8 & 0.50049 & -0.01773 & 0.254   \\
%     9 & 0.50025 & -0.01096 & 0.25222
%   \end{tabular}
%   \caption{Asymptotics for $\E \tilde{s}(\pi)$}
%   \label{tab:first_moment}
% \end{table}
Similarly, for $\partial^2_{xx} G_{T, t}(z, x) \biggr|_{x = 1}$, $P(z) = 2S^2$ and $Q(z) = (1 - S)^3$, yielding coefficients given by Table~\ref{tab:second_moment}.
\begin{table}[h]
  \centering
  \begin{tabular}{c|c|c|c|c}
    $t$ & $r$ & $d_1$ & $d_2$ & $d_3$ \\ \hline
    1 & 0.61803 & 0.63677  & -1.4661  & 0.75777 \\
    2 & 0.54369 & 0.2808   & -0.84725 & 0.47302 \\
    3 & 0.51879 & 0.11739  & -0.59    & 0.3633  \\
    4 & 0.50866 & 0.01902  & -0.45625 & 0.31131 \\
    5 & 0.50414 & -0.05008 & -0.37833 & 0.2841  \\
    6 & 0.50202 & -0.10252 & -0.3303  & 0.26915 \\
    7 & 0.50099 & -0.14322 & -0.3     & 0.26076 \\
    8 & 0.50049 & -0.17453 & -0.28081 & 0.25602 \\
    9 & 0.50025 & -0.198   & -0.26874 & 0.25334
  \end{tabular}
  \caption{Asymptotics for $\E \tilde{s}(\pi)^2$}
  \label{tab:second_moment}
\end{table}
In view of (\ref{eq:first_moment_approx}) and (\ref{eq:second_moment_approx}), the first and second moments of $\tilde{s}(\pi)$ have the asymptotics given by
\begin{align*}
  \E \tilde{s}(\pi) &\approx c_2 n r^{-n} \\
  \Var \tilde{s}(\pi) &= \E \tilde{s}(\pi)^2 - (\E \tilde{s}(\pi))^2 \\
  &\approx \left[ \left( \frac{1}{2} d_3 - c_2^2 \right) n^2 + (d_2 - 2c_1 c_2) n \right] r^{-n}
\end{align*}
% \big{COMMENTED}
%
% This means that the generating functions for $Per(A_n), Per(B_n)$, and $Per(C_n)$ have the closed forms
% \begin{align*}
%   G^A(x, y, z) &= \frac{1}{1 - xz - xz^2 - \cdots - xz^t - xyz^{t+1}} \\
%   G^B(x, z) &= \frac{1}{1 - xz - xz^2 - \cdots - xz^t - xz^{t+1}} \\
%   G^C(x, z) &= \frac{1}{1 - z - z^2 - \cdots - z^t - xz^{t+1}}
% \end{align*}
% \subsubsection{Asymptotics of $G^A$}
% Taking the derivative with respect to $x$ and $y$ gives us
% \[G^A_{xy}(x, y, z) = \frac{(1 + S)z^{t + 1}}{(1 - S)^3},\]
% where $S = z + z^2 + \cdots + z^t$. When restricting to $x = y = 1$, $G_{xy}$ is then the generating function
% \[G^A_{xy}(x, y, z) \biggr|_{x = y = 1} = \sum_{n = 0}^\infty z^n \sum_{i, j} ij C_{ij} = \sum_{n = 0}^\infty z^n F_{n+1}^{(t)} \E (C(\pi) C_{t + 1}(\pi)).\]
% The denominator $1 - S$ has a single positive real root $r$ which happens to be the root of largest magnitude. Thus $(1 - S)^3$ has a triple root at $r$, so $G_{xy} \biggr|_{x = y = 1}$ has asymptotics given by a three-term partial fraction decomposition
% \[[z^n] G^A_{xy} \biggr|_{x = y = 1} \approx [z^n] \left\{ \frac{c_1}{1 - z/r} + \frac{c_2}{(1 - z/r)^2} + \frac{c_3}{(1 - z/r)^3} \right\}.\]
% The coefficient of $z^n$ in the large-$n$ limit is therefore
% \[\left( c_1 + c_2 n + \frac{c_3 n(n + 1)}{2} \right) r^{-n}.\]
% We next compute $c_i$ using the formula
% \[c_i = -\frac{1}{r^i(3 - i)!} \lim_{z \rightarrow r} \frac{d^{3 - i}}{dz^{3 - i}} \left( (z - r)^3 G_{xy} \biggr|_{x = y = 1} \right).\]
% Generally, if $f(x) = \frac{P(x)}{Q(x)}$ and $Q(x) = (x - r)^k R(x)$, where $P, Q$, and $R$ are polynomials such that $R(r) \ne 0$, then
% \begin{align*}
%   \frac{d}{dx} \left( (x - r)^k f(x) \right) &= \left( \frac{P'}{R} - \frac{PR'}{R^2} \right) \biggr|_{x = r} \\
%   \frac{d^2}{dx^2} \left( (x - r)^k f(x) \right) &= \left( \frac{P''}{R} - \frac{PR''}{R^2} - \frac{2P' R'}{R^2} + \frac{2P(R')^2}{R^3} \right) \biggr|_{x = r}.
% \end{align*}
% Using $P = (1 + S)z^{t + 1}$ and $Q = (1 - S)^3$, we see that, in the limit $z \rightarrow r$,
% \begin{align*}
%   P &= 2r^{t + 1} \\
%   P' &= S' r^{t + 1} + 2(t+1) r^t \\
%   P'' &= S'' r^{t + 1} + 2S'(t+1) r^t + 2(t+1)t r^{t - 1} \\
%   R &= -(S')^3 \\
%   R' &= \frac{3}{2} S' \cdot S'' \\
%   R'' &= 2S' \cdot S''' + \frac{3}{4} (S'')^2
% \end{align*}
% This gives the following table of values for $c_1, c_2, c_3$, and $r$:
% \begin{table}[h]
%   \begin{tabular}{c|c|c|c|c}
%     t & r & c_1 & c_2 & c_3 \\ \hline
%     1 & 0.61803 & 0.23155 & -0.53889 & 0.28944 \\
%     2 & 0.54369 & 0.10711 & -0.17984 & 0.07602 \\
%     3 & 0.51879 & 0.06514 & -0.0783  & 0.02632 \\
%     4 & 0.50866 & 0.04429 & -0.03898 & 0.0106  \\
%     5 & 0.50414 & 0.03118 & -0.02079 & 0.00466 \\
%     6 & 0.50202 & 0.02192 & -0.01146 & 0.00216 \\
%     7 & 0.50099 & 0.01512 & -0.00641 & 0.00103 \\
%     8 & 0.50049 & 0.01017 & -0.00359 & 0.0005  \\
%     9 & 0.50025 & 0.00667 & -0.00201 & 0.00025
%   \end{tabular}
% \end{table}
%
% \subsubsection{Asymptotics of $G^B$ and $G^C$}
% We use the same approach as the previous section. We have
% \begin{align*}
%   G^B_x \biggr|_{x = 1} &= \frac{S}{(1 - S)^2} \\
%   G^B_{xx} \biggr|_{x = 1} &= \frac{S^2}{(1 - S)^3}
% \end{align*}
% As with $G^A$, we let $r$ denote the unique positive real root of $1 - S$. Then, asympotitically, we have
% \[G^B_x \sim \frac{c_1}{1 - z/r} + \frac{c_2}{(1 - z/r)^2},\]
% with constants $c_1$ and $c_2$ shown in the following table: \\
% \begin{table}[h]
%   \begin{tabular}{c|c|c|c}
%     t & r & c_1 & c_2 \\ \hline
%     1 & 0.61803 & -0.43416 & 0.52361 \\
%     2 & 0.54369 & -0.25053 & 0.38244 \\
%     3 & 0.51879 & -0.15848 & 0.32074 \\
%     4 & 0.50866 & -0.10341 & 0.28936 \\
%     5 & 0.50414 & -0.06777 & 0.27225 \\
%     6 & 0.50202 & -0.04403 & 0.26261 \\
%     7 & 0.50099 & -0.02818 & 0.25712 \\
%     8 & 0.50049 & -0.01773 & 0.254   \\
%     9 & 0.50025 & -0.01096 & 0.25222
%   \end{tabular}
% \end{table}
% For $G^B_{xx}$, we have similarly
% \[G^B_{xx} \sim \frac{d_1}{1 - z/r} + \frac{d_2}{(1 - z/r)^2} + \frac{d_3}{(1 - z/r)^3}\]
% with \\
% \begin{table}[h]
%   \begin{tabular}{c|c|c|c|c}
%     t & r & d_1 & d_2 & d_3 \\ \hline
%     1 & 0.61803 & 0.31839  & -0.73305 & 0.37889 \\
%     2 & 0.54369 & 0.1404   & -0.42362 & 0.23651 \\
%     3 & 0.51879 & 0.05869  & -0.295   & 0.18165 \\
%     4 & 0.50866 & 0.00951  & -0.22812 & 0.15566 \\
%     5 & 0.50414 & -0.02504 & -0.18917 & 0.14205 \\
%     6 & 0.50202 & -0.05126 & -0.16515 & 0.13458 \\
%     7 & 0.50099 & -0.07161 & -0.15    & 0.13038 \\
%     8 & 0.50049 & -0.08727 & -0.1404  & 0.12801 \\
%     9 & 0.50025 & -0.099   & -0.13437 & 0.12667
%   \end{tabular}
% \end{table} \\
% %TODO: Insert table for G^B_{xx}
% Since $G^B_{xx}$ has the expansion
% \[G^B_{xx} &= \sum_{n = 0}^\infty z^n \sum_{k = 0}^n k(k - 1) N_{n, k},\]
% where $N_{n, k}$ is the number of type $(t, 1)$ permutations with $k$ cycles, we see that the second moment of $C(\pi)$ is proportional to $[z^n]G^B_{xx} + [z^n] G^B_x$. In terms of the computed constants $c_1, c_2, d_1, d_2$, and $d_3$, we have
% \begin{align*}
%   [z^n] G^B_{xx} + [z^n] G^B_x &= \left( d_1 + d_2n + \frac{d_3 n(n+1)}{2} + c_1 + c_2n \right) r^{-n} \\
%   &= \left( d_1 + c_1 + (d_2 + c_2) n + \frac{d_3 n(n+1)}{2} \right) r^{-n}
% \end{align*}
% \subsubsection{Asymptotics of $G^C$}
% We have
% \begin{align*}
%   G^C(x, z)_x \biggr|_{x = 1} &= \frac{z^{t + 1}}{(1 - S)^2} \\
%   G^C(x, z)_{xx} \biggr|_{x = 1} &= \frac{2z^{2t + 2}}{(1 - S)^3}
% \end{align*}
% \begin{table}[h]
%   \begin{tabular}{c|c|c|c}
%     t & r & c_1 & c_2 \\ \hline
%     1 & 0.61803 & -0.28944 & 0.2 \\
%     2 & 0.54369 & -0.12527 & 0.06146 \\
%     3 & 0.51879 & -0.06339 & 0.02323 \\
%     4 & 0.50866 & -0.03447 & 0.00985 \\
%     5 & 0.50414 & -0.01936 & 0.00447 \\
%     6 & 0.50202 & -0.01101 & 0.00211 \\
%     7 & 0.50099 & -0.00626 & 0.00102 \\
%     8 & 0.50049 & -0.00355 & 0.0005  \\
%     9 & 0.50025 & -0.00199 & 0.00025
%   \end{tabular}
% \end{table}
% \begin{table}[h]
%   \begin{tabular}{c|c|c|c|c}
%     t & r & c_1 & c_2 & c_3 \\ \hline
%     1 & 0.61803 & 0.34733 & 0.35056 & -0.11056 \\
%     2 & 0.54369 & 0.09081 & 0.05568 & -0.01222 \\
%     3 & 0.51879 & 0.02752 & 0.01161 & -0.00191 \\
%     4 & 0.50866 & 0.0089  & 0.0028  & -0.00036 \\
%     5 & 0.50414 & 0.00295 & 0.00073 & -8 \cdot 10^{-5} \\
%     6 & 0.50202 & 0.00098 & 0.0002  & -2 \cdot 10^{-5} \\
%     7 & 0.50099 & 0.00032 & 5 \cdot 10^{-5} & 0.0 \\
%     8 & 0.50049 & 0.0001  & 2 \cdot 10^{-5} & 0.0 \\
%     9 & 0.50025 & 3 \cdot 10^{-5} & 0.0 & 0.0
%   \end{tabular}
% \end{table}
% \subsection{Computing the moments of $T$}
%
% \[G_t(z, x) = \sum_{n = 0}^\infty z^n f_n(x),\]
% where $f_n(x) = \sum_k x^k \cdot \#\{\pi \in \mc{F}_{n, t, 1}: p(\pi) = 2^{-k}\}$. Note that $\E T$ and $\E T^2$ correspond to the coefficients of $z^n$ of $G_t(z, 1)$ and $G_t(z, 2)$, respectively. Also, observe that $f_n(x) = Per(A_n^{(0)})$, where
% \[A_n^{(0)} = D_n^{(t)}(1) + D_n^{(t-1)}(x) + D_n^{(t - 2)}(x) + \cdots + D_n^{(-1)}(x).\]
% Next, for $0 < k \le t$, define $A_n^{(k)}$ to be the matrix obtained by replacing the first column of $A_n^{(0)}$ by the vector $(x, x, \ldots, x, 1, 0, 0, \ldots, 0)^T$ with $t - k$ $x$'s. Then, it is easy to check that
% \[Per(A_n^{(k)}) = \begin{cases}
%   x\left[ Per(A_{n - 1}^{(0)}) + Per(A_{n - 1}^{(k + 1)}) \right] & \mbox{if~} k < t \\
%   Per(A_{n - 1}^{(0)}) & \mbox{if~} k = t
% \end{cases}\]
% This gives us the recursion
% \[f_n(x) = \sum_{k = 1}^t x^k f_{n - k}(x) + x^t f_{n - t - 1}(x).\]
% For $n \le t$, we have
% \[A_n^{(0)} = D_n^{(n)}(x) + D_n^{(n - 1)}(x) + \cdots + D_n^{(-1)}(x),\]
% so $f_n(x) = 2^{n - 1}x^{n - 1}$. This allows us to compute $G_t(z, x)$:
% \begin{align*}
%   G_t(z, x) - \sum_{n = 0}^t z^n f_n(x) &= \sum_{n = t + 1}^\infty z^n f_n(x) \\
%   &= \sum_{n = t + 1}^\infty z^n \left( \sum_{k = 1}^t x^k f_{n - k}(x) + x^t f_{n - t - 1}(x) \right) \\
%   &= \sum_{k = 1}^t \left( (xz)^k \sum_{n \ge t - k + 1} z^n f_n(x) \right) \\
%   &= \sum_{k = 1}^t (xz)^k \left( G_t(z, x) - \sum_{n \le t - k} z^n f_n(x) \right).
% \end{align*}
% Solving for $G_t(z, x)$ gives us
% \begin{align*}
%   G_t(z, x) &= \frac{\sum_{n \le t} z^n f_n(x) - \sum_{k = 1}^t (xz)^k \sum_{n \le t - k} z^n f_n(x)}{1 - xz - (xz)^2 - \cdots - (xz)^t - x^t z^{t + 1}} \\
%   &= \frac{\sum_{n \le t} 2^{n - 1}x^{n - 1}z^n - \sum_{k = 1}^t \sum_{n \le t - k} 2^{n - 1} x^{n + k - 1}z^{n + k}}{1 - xz - (xz)^2 - \cdots - (xz)^t - x^t z^{t + 1}} \\
%   &= \frac{z(1 + xz + \cdots + (xz)^t)}{1 - xz - (xz)^2 - \cdots - (xz)^t - x^t z^{t + 1}} \\
%   \Rightarrow G(z, x) = 1 + G_t(z, x) &= \frac{1 + z(1 - x) \sum_{i = 0}^{t - 1} x_i z_i}{1 - xz - x^2 z^2 - \cdots - x^t z^t - x^t z^{t + 1}} = \frac{P(x, z)}{Q(x, z)}
% \end{align*}
% The roots of $Q(x, z)$ determine the asymptotic behavior of the coefficients in its power series expansion. To that end, we write
% \[G(z, x) = \sum_i \left( \frac{a_{i1}}{z - r_i} + \frac{a_{i2}}{(z - r_i)^2} + \cdots + \frac{a_{i k_i}}{(z - r_i)^{k_i}} \right),\]
% Observe that for fixed $x \ge 1$, $Q(x, z)$ is monotonically decreasing in $z$ on the nonnegative reals, and that $p(x, 0) = 1$ and $p(x, 1) < 0$. Therefore, $p(x, z)$ has a unique positive real root. Furthermore, this root necessarily has the smallest norm among all roots, since any root $r$ satisfies $p(x, \abs{r}) \le 0$.
% We may write $G(z, x)$ as
% where $k_i$ is the multiplicity of the root $r_i$. Since $r$ is a simple root, the coefficient corresponding to $\frac{1}{z - r}$ is
% \[\frac{P(x, z)}{Q'(x, z)} = -\frac{1 + z(1 - x)\sum_{i = 0}^{t - 1} x^i z^i}{x(1 + 2xz + 3x^2 z^2 + \cdots + t x^{t - 1} z^{t - 1} + (t + 1) x^{t - 1}z^t)}.\]
% Letting $S = \sum_{i = 0}^\infty (xz)^i$, we see that in the radius of convergence,
% \subsection{Central Limit Theorems}
% In this section, we try to prove a Central Limit Theorem for the number of $(t + 1)$-cycles in a uniformly random permutation from a restriction matrix of type $(t, 1)$. This result was shown combinatorially in~\cite{dgh01} for $t = 1$ (Fibonacci permutations). \\
% Let $P_n(x) = \sum_{k = 0}^n P(k(\pi) = k) x^k$ be the probability generating function of $k(\pi)$. Then, $P_n(x)$ is proportional to $Q_n(x) = Per(A_n(x))$, with constant of proportionality equal to the number of restricted permutations of type $(t, 1)$.
% \begin{proposition}\label{prop:basic_properties}
%   Fix $t$, and let $P_n = Per(A_{n, t}(x))$. Then, $P_n$ has degree $n - 1$ and has a root at 0 of multiplicity $\ceil{\frac{t(n - 1)}{t + 1}}$.
% \end{proposition}
% \begin{proof}
%   That $P_n$ has degree $n - 1$ can be seen by induction, noting that $P_k = (2x)^{k - 1}$ has degree $k - 1$ for $k \le t + 1$. \\
%   The maximum value of $k(\pi)$ if $\pi$ is a restricted permutation of type $(t, 1)$ is $\floor{\frac{n - 1}{t + 1}}$. Therefore, every monomial in $P_n$ has degree at least $n - 1 - \floor{\frac{n - 1}{t + 1}}$, with equality coming from the permutations which attain this maximum.
% \end{proof}
% Next, we show that the roots of $P_n$ are real. Then, by [Pitman], the random variable $X$ with the probability generating function $P_n$ can be expressed as a sum of independent Bernoulli random variables, and therefore is asymptotically normal. \\
% To prove real-rootedness, we show that the roots of the $P_i$ satisfy an interlacing property.
% \begin{definition}
%   Let $f_1, \ldots, f_k$ be polynomials of degree $n$ or $n - 1$ for some integer $n > 0$. We say that $f_1, \ldots, f_k$ have \emph{common interlacing} if there exists a polynomial $g$ of degree $n - 1$ and real roots $r_1, \ldots, r_{n - 1}$ such that
% \end{definition}
% We first observe that since $P_k = (2x)^{k - 1}$ for $k \le t + 1$, the first $t + 1$ polynomials in the sequence are real-rooted.
% \begin{proposition}
%   Suppose $P_1, \ldots, P_n$ are real-rooted for some $n > t + 1$. Let $\{a_1^{(k)} \le \ldots \le a_{n - 1}^{(k)}\}$ be the ordered roots of $x^k P_{n - k}$, for each $k \le t$, and let $\{a_1^{(t + 1)} \le \ldots \le a_{n - 2}^{(t + 1)}\}$ be the roots of $x^t P_{n - t - 1}$. Then, there exist real numbers $b_1 \le \ldots \le b_{n - 1}$, which we will call $I_n$, for which $a_i^{(k)} \le b_i \le a_{i + 1}^{(k)}$ for all $i < n$ and $k \le t + 1$.
% \end{proposition}
% \begin{proof}
%   The claim is true for $n \le t + 1$ by inspection. Suppose it is true for all $n < m$, and let $I_{m - 1} = \{b_1 \le \ldots \le b_{m - 2}\}$. Then, since all of the polynomials $P_j$ have positive coefficients, the values of $\{x_k P_{m - k}\}_{k = 1}^t$ and $x^t P_{m - t - 1}$ must have the same sign at each of the values $b_i$. This means that $P_m$ changes sign between any two nonequal $b_j, b_{j + 1}$, and must therefore have a root in the interval $(b_j, b_{j + 1})$. By Proposition~\ref{prop:basic_properties}, the multiplicity of the root at 0 of $x^k P_{n - k}$ is $k + \ceil{\frac{t(n - k - 1)}{t + 1}}$. Since $P_n = xP_{n - 1} + x^2 P_{n - 2} + \cdots + x^t P_{n - t} + x^t P_{n - t - 1}$,
% \end{proof}
% %TODO: cite result from pitman that probability generating functions with real roots can be expressed as sums of Bernoullis
% \begin{lemma}
%   Let For every $n > t + 1$, the roots of $P_n(x), x P_{n - 1}(x), \ldots, x^t P_{n - t}, x^t P_{n - t - 1}(x)$ have a common interlacing. That is, there exist $a_1 \le a_2 \le \cdots, a_{n - 1} \le 0$ such that
% \end{lemma}
% The following theorem from~\cite{ms18} gives a sufficient criterion on the roots of $P_n$ in determining whether or not $k(\pi)$ satisfies a central limit theorem as $n \rightarrow \infty$.
% \begin{theorem}
%   Let $\epsilon > 0$ and, for each $n$, let $X_n \in \{0, \ldots, n\}$ be a random variable with standard deviation $\sigma_n > n^{\epsilon}$. If all the roots $\zeta$ of $P_n$ satisfy $\abs{1 - \zeta} > 1/\sigma_n^{1 - \epsilon}$, then the sequence $\{X_n\}$ satisfies a central limit theorem.
% \end{theorem}
% Since $P_n$ is proportional to $Per(A_n)$, it suffices to show that $Per(A_n)$ has roots that are bounded away from 1. In particular, we show the following:
% \begin{proposition}
%   The polynomial $Per(A_n(x))$ has all real roots. In particular, since $Per(A_n(x))$ has nonnegative real coefficients, all of its roots are on the negative real axis.
% \end{proposition}
% \begin{proof}
%   The statement is clearly true for $Per(A_1(x)) = 1$ and $Per(A_2(x)) = 2x$. In particular, for $i = 1, 2$, the real part of $Per(A_i(\zeta))$ has the same sign as the real part of $\zeta$. Using the recursion $Per(A_n(x)) = x(Per(A_{n - 1})(x) + Per(A_{n - 2})(x))$, we see that if $Re(\zeta) > 0$, then $Per(A_{n - 1}(\zeta)) + Per(A_{n - 2}(\zeta))$ must also have a positive real part. It follows that
% \end{proof}
% \subsection{KL divergence}
% The KL divergence between two distributions $\mu$ and $\nu$ is given by
% \[D_{KL}(\mu \| \nu) = \E_\mu \left( \log \frac{d\nu}{d\mu} \right).\]
% In our case, $\mu$ and $\nu$ are the uniform and sampling distributions over restricted permutations of type $(t, 1)$, respectively, so $\frac{d\nu}{d\mu}(\pi) = S_{n, t} \cdot 2^{-k'(\pi)}$, where $k(\pi) = \#\{i: \pi(i) \ne i - t\}$.
% \[D_{KL}(\mu \| \nu) = \log S_{n, t} - \log 2 \E_\mu \left( k'(\pi) \right).\]
% Next, observe that $\E_\mu k'(\pi) = \frac{1}{S_{n, t}} \sum_{0 \le k \le n - 1} k g_n(k)$, where $g_n(k)$ is the number of permutations $\pi \in S_n$ of type $(t, 1)$ satisfying $k'(\pi) = k$. In relation to the generating function $G(x, z)$, we see that
% \subsection{Counting the number of cycles}
% Write $\pi \in S_n$ as $x_1^{a_1} \cdots x_n^{a_n}$, where $a_k$ is the number of $k$-cycles in $\pi$. This means that $\sum ia_i = n$. Consider the polynomial $C_n(x_1, \ldots, x_n) = \frac{1}{n!} \sum_{\pi \in S_n} \prod_{i = 1}^n x_i^{a_i(\pi)}$, and let $C(t) = \sum_{n = 0}^\infty t^n C_n(x)$. It is then a theorem of Polya that
% \[C(t) = \exp\left( \sum_{i = 1}^\infty t^i \frac{x_i}{i} \right).\]
% Next, recall that the poisson distribution with parameter $\theta$ has probability mass function
% \[P_\theta(j) = \frac{e^{-\theta} \theta^j}{j!}.\]
% Define the polynomial
% \begin{align*}
%   M_\theta(x) &= \sum_{j = 0}^\infty x^j P_\theta(j) \\
%   &= \sum_{j = 1}^\infty \frac{x^j \theta^j e^{-\theta}}{j!} \\
%   &= e^{-\theta + x\theta}.
% \end{align*}
% Consider the case of computing the number of cycles $C(\pi) = \sum_{i = 1}^n a_i$. Setting all $x_i$ to be the same, we have $C_n(x, t) = \frac{1}{n!} \sum_{\pi \in S_n} x^{C(\pi)}$. This represents the expected value of $x^{C(\pi)}$ where $\pi$ is drawn uniformly from $S_n$. Associated with $C_n$ is the quantity
% \[C(x, t) = \sum_{n = 0}^\infty t^n C_n(t) = \exp\left( x\sum_{i = 1}^\infty \frac{t^i}{i} \right) = \exp(-x \log(1 - t)) = \frac{1}{(1 - t)^x}.\]
% Next, we use the expansion
% \[(1 - t)^{-x} = \sum_{j = 0}^\infty \frac{\Gamma(-x)}{\Gamma(-x - j) j!} (-t)^j,\]
% giving us
% \[\sum_{n = 0}^\infty t^n C_n(x, t) = \sum_{j = 0}^\infty \frac{(x + 1)\cdots (x + j - 1)}{j!} t^j.\]
% Matching coefficients, we see that $C_n(x, t) = \prod_{i = 2}^n \left( \frac{i - 1}{i} + \frac{x}{i} \right)$. To interpret these results, let $\{X_i\}$ denote an independent collection of Bernoulli random variables with parameters $1/i$.

